Modeling non-linear spectral domain dependence using copulas with applications to rat local field potentials

This paper intends to develop tools for characterizing non-linear spectral dependence between spontaneous brain signals. We use parametric copula models (both bivariate and vine models) applied on the magnitude of Fourier coefficients rather than using coherence. The motivation behind this work is an experiment on rats that studied the impact of stroke on the connectivity structure (dependence) between local field potentials recorded at various channels. We address the following major questions. First, we ask whether one can detect any changepoint in the regime of a brain channel for a given frequency band based on a difference between the cumulative distribution functions modeled for each epoch (small window of time). Our proposed approach is an iterative algorithm which compares each successive bivariate copulas on all the epochs range, using a bivariate Kolmogorov-Smirnov statistic. Second, we ask whether stroke can alter the dependence structure of brain signals; and examine whether changes in dependence are present only in some channels or generalized across channels. These questions are addressed by comparing Vine-copulas models fitted for each epoch. We provide the necessary framework and show the effectiveness of our methods through the results for the local field potential data analysis of a rat.

==> ChangepointsForRats150326to160406.tex <==
\begin{table}{\footnotesize
\begin{tabular}{|l||*{1}{c|c|}} 

    \hline
     \textbf{Channel and} & Copula-based &  Condordance with    \\
		 \textbf{Frequency band}    & algorithm & James algorithm \\
    \hline \hline
    Channel 1, $\Delta$ &$287,300,301$ \\ 
		Channel 1, $\theta$ &$\*$(\textit{46 changepoints have been detected})  \\ 
		Channel 1, $\alpha$ &$\*$(\textit{40 changepoints have been detected})  \\
		Channel 1, $\beta$ &$72,73,81,128,210,273,274,275$  \\
		Channel 1, $\gamma$ &$\*$(\textit{27 changepoints have been detected})  \\
		\hline
		Channel 9, $\Delta$ &$293,301,423,544$ \\ 
		Channel 9, $\theta$ &$\*$(\textit{43 changepoints have been detected})  \\
		Channel 9, $\alpha$ & $\*$(\textit{83 changepoints have been detected})  \\
		Channel 9, $\beta$ &$\*$(\textit{39 changepoints have been detected}) \\
		Channel 9, $\gamma$ &  $\*$(\textit{20 changepoints have been detected})  \\
		\hline
	  Channel 17, $\Delta$ &$26,27,56,190,193,260$  \\
		Channel 17, $\theta$ & $26,27,56,131,132,134,202,203,293$ \\
		Channel 17, $\alpha$ &$26,69,131,132,175,176,202,203,293$  \\
		Channel 17, $\beta$ & $\*$(\textit{46 changepoints have been detected})  \\
		Channel 17, $\gamma$ &$26,27,69,70,79,131,175,176,203,293$  \\
		\hline 
		   \end{tabular}}

	\caption{Epochs considered as changepoints using the copula-based algorithm (with a threshold of $\bar{\alpha}=1\%$), for rat id $150326$.  }
	\label{changeEpochs}

\end{table}

\begin{table}{\footnotesize
\begin{tabular}{|l||*{1}{c|c|}} 

    \hline
     \textbf{Channel and} & Copula-based &  Condordance with    \\
		 \textbf{Frequency band}    & algorithm & James algorithm \\
    \hline \hline
    Channel 1, $\Delta$ &$525,526,549$ \\ 
		Channel 1, $\theta$ &$\*$(\textit{20 changepoints have been detected})  \\ 
		Channel 1, $\alpha$ &$\*$(\textit{42 changepoints have been detected})  \\
		Channel 1, $\beta$ &(\textit{42 changepoints have been detected})  \\
		Channel 1, $\gamma$ &$\*$(\textit{25 changepoints have been detected})  \\
		\hline
		Channel 9, $\Delta$ &$315,317,525,526,529,533,549$ \\ 
		Channel 9, $\theta$ &$\*$(\textit{23 changepoints have been detected})  \\
		Channel 9, $\alpha$ & $\*$(\textit{49 changepoints have been detected})  \\
		Channel 9, $\beta$ &$\*$(\textit{39 changepoints have been detected}) \\
		Channel 9, $\gamma$ &  $\*$(\textit{25 changepoints have been detected})  \\
		\hline
	  Channel 17, $\Delta$ &$315,317,525,526,529,533,538,548,549$  \\
		Channel 17, $\theta$ & $\*$(\textit{34 changepoints have been detected}) \\
		Channel 17, $\alpha$ &$\*$(\textit{41 changepoints have been detected})  \\
		Channel 17, $\beta$ & $\*$(\textit{32 changepoints have been detected})  \\
		Channel 17, $\gamma$ &$\*$(\textit{25 changepoints have been detected})  \\
		\hline 
		   \end{tabular}}

	\caption{Epochs considered as changepoints using the copula-based algorithm (with a threshold of $\bar{\alpha}=1\%$), for rat id $150410$.  }
	\label{changeEpochs}

\end{table}


==> Tables4Rats.tex <==
\begin{table}[h]
\begin{center}
{\tiny \begin{tabular}{|l||*{8}{c|}}

        \cline{2-9} 
				\multicolumn{1}{c|}{} & & & & & & & & \\
      \multicolumn{1}{c|}{} & Channel 1  & Channel 2  & Channel 9 & Channel 10 & Channel 17 & Channel 18  & Channel  25 & Channel 26 \\
    \hline \hline
    Channel 1  & \cellcolor{intnull} & $270$ & $270$ & $270$ & $270$ & $270$ & $270$ & $270$ \\
		           & \cellcolor{intnull} & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$  & $p<0.0001$ &$p<0.0001$ \\ \hline
							
    Channel 2  & $270$ & \cellcolor{intnull} & $17$ & $20$& $266$ & $46$ & $266$& $268$ \\
             & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ \\ \hline	
										
    Channel 9  &$270$ & $17$ & \cellcolor{intnull} & $250$  & $262$ & $260$ & $265$ & $264$\\
		           &$p<0.0001$ & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$\\ \hline
							
    Channel 10  & $270$ & $20$& $250$ & \cellcolor{intnull} & $262$ & $159$ & $267$ & $267$ \\
             & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$ & $p=0.004$ & $p<0.0001$ & $p<0.0001$ \\ \hline	
						
    Channel 17  & $270$ & $266$ & $262$ & $262$ & \cellcolor{intnull}& $13$ &$76$ & $262$\\
		           & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$& $ p<0.0001$& $p<0.0001$ \\ \hline
							
    Channel 18  & $270$ & $46$ &$260$ &$159$ & $13$ & \cellcolor{intnull} & $264$ & $264$ \\
             & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p=0.004$ & $p<0.0001$ & \cellcolor{intnull} & $p < 0.0001$ & $p < 0.0001$ \\ \hline	
						
    Channel 25  & $270$ & $266$ & $265$ & $267$ & $76$& $264$ & \cellcolor{intnull} & $256$\\
		           & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p < 0.0001$ & \cellcolor{intnull} & $p < 0.0001$ \\ \hline
							
    Channel 26  & $270$ & $268$ &$264$ & $267$ & $262$ & $264$ & $256$ & \cellcolor{intnull} \\
             & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p < 0.0001$ & $p < 0.0001$ & \cellcolor{intnull}\\ \hline							

		\hline
		  \end{tabular}}
	\caption{RAT 150326 }
	\label{changeChannels}
\end{center}
\end{table}



\begin{table}[h]
\begin{center}
{\tiny \begin{tabular}{|l||*{8}{c|}}

        \cline{2-9} 
				\multicolumn{1}{c|}{} & & & & & & & & \\
      \multicolumn{1}{c|}{} & Channel 1  & Channel 2  & Channel 9 & Channel 10 & Channel 17 & Channel 18  & Channel  25 & Channel 26 \\
    \hline \hline
    Channel 1  & \cellcolor{intnull} & $ 1$ & $1 $ & $ 184$ & $251 $ & $270 $ & $247 $ & $79 $ \\
		           & \cellcolor{intnull} & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$  & $p<0.0001$ &$p<0.0001$ \\ \hline
							
    Channel 2  & $ 1$ & \cellcolor{intnull} & $242$ & $233$& $259 $ & $265$ & $250$& $178$ \\
             & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ \\ \hline	
										
    Channel 9  &$1 $ & $242$ & \cellcolor{intnull} & $219$  & $270$ & $270$ & $268$ & $269$\\
		           &$p<0.0001$ & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$\\ \hline
							
    Channel 10  & $184 $ & $233$& $219$ & \cellcolor{intnull} & $250$ & $270$ & $232$ & $75$ \\
             & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$ & $p>0.001$ & $p<0.0001$ & $p<0.0001$ \\ \hline	
						
    Channel 17  & $251 $ & $259 $ & $270$ & $250$ & \cellcolor{intnull}& $204$ &$166$ & $12$\\
		           & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$& $ p=0.0002$& $p<0.0001$ \\ \hline
							
    Channel 18  & $270 $ & $265$ &$270$ &$270$ & $204$ & \cellcolor{intnull} & $96$ & $14$ \\
             & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p>0.001$ & $p<0.0001$ & \cellcolor{intnull} & $p < 0.0001$ & $p < 0.0001$ \\ \hline	
						
    Channel 25  & $ 247 $ & $250$ & $268$ & $232$ & $166$& $96$ & \cellcolor{intnull} & $14$\\
		           & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p=0.0002$ & $p < 0.0001$ & \cellcolor{intnull} & $p < 0.0001$ \\ \hline
							
    Channel 26  & $79 $ & $178$ &$269$ & $75$ & $12$ & $14$ & $14$ & \cellcolor{intnull} \\
             & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p < 0.0001$ & $p < 0.0001$ & \cellcolor{intnull}\\ \hline							

		\hline
		  \end{tabular}}
	\caption{RAT 150410 }
	\label{changeChannels}
\end{center}
\end{table}





\begin{table}[h]
\begin{center}
{\tiny \begin{tabular}{|l||*{8}{c|}}

        \cline{2-9} 
				\multicolumn{1}{c|}{} & & & & & & & & \\
      \multicolumn{1}{c|}{} & Channel 1  & Channel 2  & Channel 9 & Channel 10 & Channel 17 & Channel 18  & Channel  25 & Channel 26 \\
    \hline \hline
    Channel 1  & \cellcolor{intnull} & $ 1$ & $1 $ & $ 184$ & $251 $ & $270 $ & $247 $ & $79 $ \\
		           & \cellcolor{intnull} & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$  & $p<0.0001$ &$p<0.0001$ \\ \hline
							
    Channel 2  & $ 1$ & \cellcolor{intnull} & $242$ & $233$& $259 $ & $265$ & $250$& $178$ \\
             & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ \\ \hline	
										
    Channel 9  &$1 $ & $242$ & \cellcolor{intnull} & $219$  & $270$ & $270$ & $268$ & $269$\\
		           &$p<0.0001$ & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$\\ \hline
							
    Channel 10  & $184 $ & $233$& $219$ & \cellcolor{intnull} & $250$ & $270$ & $232$ & $75$ \\
             & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$ & $p>0.001$ & $p<0.0001$ & $p<0.0001$ \\ \hline	
						
    Channel 17  & $251 $ & $259 $ & $270$ & $250$ & \cellcolor{intnull}& $204$ &$166$ & $12$\\
		           & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & \cellcolor{intnull} & $p<0.0001$& $ p=0.0002$& $p<0.0001$ \\ \hline
							
    Channel 18  & $270 $ & $265$ &$270$ &$270$ & $204$ & \cellcolor{intnull} & $96$ & $14$ \\
             & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p>0.001$ & $p<0.0001$ & \cellcolor{intnull} & $p < 0.0001$ & $p < 0.0001$ \\ \hline	
						
    Channel 25  & $ 247 $ & $250$ & $268$ & $232$ & $166$& $96$ & \cellcolor{intnull} & $14$\\
		           & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p=0.0002$ & $p < 0.0001$ & \cellcolor{intnull} & $p < 0.0001$ \\ \hline
							
    Channel 26  & $79 $ & $178$ &$269$ & $75$ & $12$ & $14$ & $14$ & \cellcolor{intnull} \\
             & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p<0.0001$ & $p < 0.0001$ & $p < 0.0001$ & \cellcolor{intnull}\\ \hline							

		\hline
		  \end{tabular}}
	\caption{RAT 160406}
	\label{changeChannels}
\end{center}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!htbp]
{\tiny 
$$
\begin{pmatrix}
    \begin{smallmatrix} {\color{blue}1} \\ \begin{pmatrix} 1 \\ p < 0.0001 \end{pmatrix}  \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}2} \\ \begin{pmatrix} 50 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}3} \\ \begin{pmatrix} 22 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}4} \\ \begin{pmatrix} 132 \\ {\color{red} p=0.7610} \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}5} \\ \begin{pmatrix} 1 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}6} \\ \begin{pmatrix} 51 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}7} \\ \begin{pmatrix} 34 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}8} \\ \begin{pmatrix} 56 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix}
		\\ & & & & & & & \\
    \begin{smallmatrix} {\color{blue}9} \\ \begin{pmatrix} 1 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}10} \\ \begin{pmatrix} 41 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}11} \\ \begin{pmatrix} 1 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}12} \\ \begin{pmatrix} 10 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}13} \\ \begin{pmatrix} 33 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}14} \\ \begin{pmatrix} 117 \\  {\color{red} p=0.03297}  \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}15} \\ \begin{pmatrix} 32 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}16} \\ \begin{pmatrix} 5 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix}
		\\ & & & & & & & \\
    \begin{smallmatrix} {\color{blue}17} \\ \begin{pmatrix} 53 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}18} \\ \begin{pmatrix} 13 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}19} \\ \begin{pmatrix} 5 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}20} \\ \begin{pmatrix} 16 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}21} \\ \begin{pmatrix} 25 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}22} \\ \begin{pmatrix} 35 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}23} \\ \begin{pmatrix} 56 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}24} \\ \begin{pmatrix} 28 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix}
		\\ & & & & & & &\\		
	  \begin{smallmatrix} {\color{blue}25} \\ \begin{pmatrix} 20 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}26} \\ \begin{pmatrix} 6 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}27} \\ \begin{pmatrix} 1 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}28} \\ \begin{pmatrix} 1 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}29} \\ \begin{pmatrix} 60 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}30} \\ \begin{pmatrix} 36 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}31} \\ \begin{pmatrix} 7 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}32} \\ \begin{pmatrix} 1 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix}
		
\end{pmatrix}
$$
 }
\caption{RAT 150326}
\label{   }
\end{figure}

\begin{figure}[!htbp]
{\tiny 
$$
\begin{pmatrix}
    \begin{smallmatrix} {\color{blue}1} \\ \begin{pmatrix} 269 \\ p < 0.0001 \end{pmatrix}  \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}2} \\ \begin{pmatrix} 266 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}3} \\ \begin{pmatrix} 268 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}4} \\ \begin{pmatrix} 267 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}5} \\ \begin{pmatrix} 266 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}6} \\ \begin{pmatrix} 267 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}7} \\ \begin{pmatrix} 267 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}8} \\ \begin{pmatrix} 266 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix}
		\\ & & & & & & & \\
    \begin{smallmatrix} {\color{blue}9} \\ \begin{pmatrix} 268 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}10} \\ \begin{pmatrix} 269 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}11} \\ \begin{pmatrix} 264 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}12} \\ \begin{pmatrix} 267 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}13} \\ \begin{pmatrix} 268 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}14} \\ \begin{pmatrix} 267 \\  p< 0.0001  \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}15} \\ \begin{pmatrix} 265 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}16} \\ \begin{pmatrix} 265 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix}
		\\ & & & & & & & \\
    \begin{smallmatrix} {\color{blue}17} \\ \begin{pmatrix} 265 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}18} \\ \begin{pmatrix} 268 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}19} \\ \begin{pmatrix} 266 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}20} \\ \begin{pmatrix} 269 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}21} \\ \begin{pmatrix} 267 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}22} \\ \begin{pmatrix} 264 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}23} \\ \begin{pmatrix} 263 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}24} \\ \begin{pmatrix} 268 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix}
		\\ & & & & & & &\\		
	  \begin{smallmatrix} {\color{blue}25} \\ \begin{pmatrix} 256 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}26} \\ \begin{pmatrix} 267 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}27} \\ \begin{pmatrix} 261 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}28} \\ \begin{pmatrix} 265 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}29} \\ \begin{pmatrix}  266 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}30} \\ \begin{pmatrix} 269 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}31} \\ \begin{pmatrix} 268 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}32} \\ \begin{pmatrix} 270 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix}
		
\end{pmatrix}
$$
 }
\caption{RAT 150410}
\label{   }
\end{figure}


\begin{figure}[!htbp]
{\tiny 
$$
\begin{pmatrix}
    \begin{smallmatrix} {\color{blue}1} \\ \begin{pmatrix} 201 \\ p < 0.0001 \end{pmatrix}  \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}2} \\ \begin{pmatrix} 177  \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}3} \\ \begin{pmatrix}  245 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}4} \\ \begin{pmatrix} 254  \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}5} \\ \begin{pmatrix}  249 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}6} \\ \begin{pmatrix}  221 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}7} \\ \begin{pmatrix} 213  \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}8} \\ \begin{pmatrix}  222 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix}
		\\ & & & & & & & \\
    \begin{smallmatrix} {\color{blue}9} \\ \begin{pmatrix}  232 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}10} \\ \begin{pmatrix} 145  \\ {\color{red}p=0.2475} \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}11} \\ \begin{pmatrix} 218  \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}12} \\ \begin{pmatrix}  175 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}13} \\ \begin{pmatrix}   \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}14} \\ \begin{pmatrix} 189  \\  p< 0.0001  \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}15} \\ \begin{pmatrix} 200  \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}16} \\ \begin{pmatrix} 223  \\ p< 0.0001 \end{pmatrix} \end{smallmatrix}
		\\ & & & & & & & \\
    \begin{smallmatrix} {\color{blue}17} \\ \begin{pmatrix} 195 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}18} \\ \begin{pmatrix} 176 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}19} \\ \begin{pmatrix} 148 \\ {\color{red}p = 0.1280} \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}20} \\ \begin{pmatrix} 140 \\ {\color{red}p = 0.5840} \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}21} \\ \begin{pmatrix} 174 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}22} \\ \begin{pmatrix} 181 \\ p< 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}23} \\ \begin{pmatrix} 126 \\ {\color{red}p = 0.3009} \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}24} \\ \begin{pmatrix} 210 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix}
		\\ & & & & & & &\\		
	  \begin{smallmatrix} {\color{blue}25} \\ \begin{pmatrix} 143 \\ {\color{red}p = 0.3613} \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}26} \\ \begin{pmatrix} 142 \\ {\color{red}p = 0.4289} \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}27} \\ \begin{pmatrix} 144 \\ {\color{red}p = 0.3009} \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}28} \\ \begin{pmatrix} 81 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}29} \\ \begin{pmatrix}  160 \\ p=0.0028 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}30} \\ \begin{pmatrix} 163 \\ p=0.0008 \end{pmatrix} \end{smallmatrix} & 
		\begin{smallmatrix} {\color{blue}31} \\ \begin{pmatrix} 108 \\ p =0.0012 \end{pmatrix} \end{smallmatrix} &
		\begin{smallmatrix} {\color{blue}32} \\ \begin{pmatrix} 191 \\ p < 0.0001 \end{pmatrix} \end{smallmatrix}
		
\end{pmatrix}
$$
 }
\caption{RAT 160406}
\label{   }
\end{figure}

